Multiclass Transductive Online Learning

We consider the problem of multiclass transductive online learning when the number of labels can be unbounded. Previous works by Ben-David et al. [1997] and Hanneke et al. [2023b] only consider the case of binary and finite label spaces, respectively. The latter work determined that their techniques fail to extend to the case of unbounded label spaces, and they pose the question of characterizing the optimal mistake bound for unbounded label spaces. We answer this question by showing that a new dimension, termed the Level-constrained Littlestone dimension, characterizes online learnability in this setting. Along the way, we show that the trichotomy of possible minimax rates of the expected number of mistakes established by Hanneke et al. [2023b] for finite label spaces in the realizable setting continues to hold even when the label space is unbounded. In particular, if the learner plays for $T \in \mathbb{N}$ rounds, its minimax expected number of mistakes can only grow like $\Theta(T)$, $\Theta(\log T)$, or $\Theta(1)$. To prove this result, we give another combinatorial dimension, termed the Level-constrained Branching dimension, and show that its finiteness characterizes constant minimax expected mistake-bounds. The trichotomy is then determined by a combination of the Level-constrained Littlestone and Branching dimensions. Quantitatively, our upper bounds improve upon existing multiclass upper bounds in Hanneke et al. [2023b] by removing the dependence on the label set size. In doing so, we explicitly construct learning algorithms that can handle extremely large or unbounded label spaces. A key and novel component of our algorithm is a new notion of shattering that exploits the sequential nature of transductive online learning. Finally, we complete our results by proving expected regret bounds in the agnostic setting, extending the result of Hanneke et al. [2023b].

==> Main/Trichotomy_neurips.tex <==

% Vinod and Unique.

\section{A Trichotomy in the Realizable Setting} \label{Trichotomy}

We start by establishing upper and lower bounds on the minimax expected number of mistakes in the realizable setting in terms of the Level-constrained Littlestone dimension and the Level-constrained Branching dimension. 


\begin{theorem} [Mistake bound] \label{thm:mistakebnd} For every concept class $\mathcal{C} \subseteq \Ycal^{\Xcal}$, we have
\[\frac{1}{2} \min\Big\{\max \Big\{\operatorname{D}(\mathcal{C}), \floor{\log{T}}\, \cdot \mathbbm{1}[\operatorname{B}(\mathcal{C}) = \infty]  \Big\}, T \Big\}\,  \leq \, \operatorname{M}^{\star}(T, \mathcal{C})\, \leq \,  \min \left\{ \operatorname{B}(\mathcal{C}),  \operatorname{D}(\mathcal{C}) \, \log \left(\frac{eT}{\operatorname{D}(\mathcal{C})} \right),  T \right\}. \]
\end{theorem}

\noindent One can trivially upper bound $\operatorname{M}^{\star}(T, \mathcal{C})$ by $\operatorname{L(\mathcal{C})}$. However, by Proposition \ref{prop:relations}, our upper bound in terms of $\operatorname{B}(\mathcal{C})$ is sharper. We can also infer from the proof in Section \ref{sec:logTlb} that when $T$ is large enough (namely $T \gg 2^{\operatorname{B}(\mathcal{C})})$, the lower bound in the realizable setting is also $\frac{\operatorname{B}(\mathcal{C})}{2}$. 

Given Theorem \ref{thm:mistakebnd}, we immediately infer a trichotomy in minimax rates. 
\begin{corollary} [Trichotomy]\label{cor:trichotomy} For every concept class $\mathcal{C} \subseteq \Ycal^{\Xcal}$, we have

$$
\operatorname{M}^{\star}(T, \mathcal{C})=\begin{cases}
			\Theta(1), & \text{if $\operatorname{B}(\mathcal{C}) < \infty.$}\\
            \Theta(\log T) & \text{if $\operatorname{D}(\mathcal{C}) < \infty$ and  $\operatorname{B}(\mathcal{C}) = \infty$.}\\
            \Theta(T), & \text{if } \operatorname{D}(\mathcal{C}) =  \infty.
		 \end{cases}
$$
\end{corollary}
\begin{proof}(of Corollary \ref{cor:trichotomy}) When $\operatorname{B}(\mathcal{C}) < \infty$, Theorem \ref{thm:mistakebnd} gives that $\frac{1}{2} \operatorname{D}(\mathcal{C})\leq \operatorname{M}^{\star}(T, \mathcal{C}) \leq \operatorname{B}(\mathcal{C})$ for $T \geq \operatorname{D}(\mathcal{C})$. When $\operatorname{B}(\mathcal{C}) = \infty$ but $\operatorname{D}(\mathcal{C}) < \infty$, Theorem \ref{thm:mistakebnd} gives that $\frac{1}{2}\, \floor{\log{T}}\, \leq \operatorname{M}^{\star}(T, \mathcal{C}) \leq \operatorname{D}(\mathcal{C}) \log \Bigl(\frac{eT}{\operatorname{D}(\mathcal{C})} \Bigl)$ for $\floor{\log{T}} \geq \operatorname{D}(\mathcal{C})$. Finally, when $\operatorname{D}(\mathcal{C}) = \infty$, Theorem \ref{thm:mistakebnd} gives that $\frac{T}{2}\leq  \operatorname{M}^{\star}(T, \mathcal{C}) \leq T$. 
\end{proof}

The remainder of this Section is dedicated to proving Theorem \ref{thm:mistakebnd}. The proof of the lowerbound $\operatorname{D}(\mathcal{C})/2$  follows from standard techniques, so we defer it to Appendix \ref{app:lb_DC}.

\subsection{Proof of Upperbound $\operatorname{B}(\mathcal{C})$}
\begin{proof}
    Fix $n \in \mathbb{N}$, a sequence of instances $x_{1:n}: = (x_1, \ldots, x_n) \in \Xcal^n$, a sequence of functions $Y_{1:n} = (Y_1, \ldots, Y_n)$ such that $Y_{t}: \{0,1\}^n \to \Ycal$, and set of concepts $V \subseteq \mathcal{C}$. If $\forall \sigma \in \{0,1\}^n$, there exists $c_{\sigma } \in V$  such that $c_{\sigma}(x_t) = Y_{t}(\sigma_{\leq t})$ for all $t \in [n]$, then define $\operatorname{B}(V, x_{1:n}, Y_{1:n}) := 
    \argmin_{\sigma \in \{0,1\}^n } \sum_{t=1}^n \mathbbm{1}\{Y_{t}((\sigma_{<t}, 0)) \neq Y_{t}((\sigma_{<t}, 1)).$
 Otherwise, define $\operatorname{B}(V, x_{1:n}, Y_{1:n}):= 0$. Recall that we can represent $x_{1:n}$ and $Y_{1:n}$ with level-constrained trees $\Tcal$ of depth $n$. With the tree representation, $\operatorname{B}(V, x_{1:n}, Y_{1:n}):= 0$ if $V$ does not shatter $\Tcal$. If $\Tcal$ is shattered by $V$, then $\operatorname{B}(V, x_{1:n}, Y_{1:n})$ is the minimum branching factor across all the root-to-leaf paths in $\Tcal$. Recall that the branching factor of a path is the number of nodes in this path whose left and right outgoing edges are labeled by two distinct elements of $\Ycal$. 
In this proof, we work with an instance-dependent complexity measure of $V \subseteq \mathcal{C}$ defined as
\[\operatorname{B}(V, x_{1:n}) := \, \sup_{Y_{1:n}}\, \operatorname{B}(V, x_{1:n}, Y_{1:n}). \]




We now define a learning algorithm that obtains the claimed mistake bound of $\operatorname{B}(\mathcal{C})$. Fix a time horizon $T \in \mathbb{N}$, and let $x_{1:T} = (x_1, x_2, \ldots, x_T)$ denote the sequence of instances revealed by the adversary. Initialize $V_1 := \mathcal{C}$. For every $t \in \{1, \ldots, T\}$, if we have $\{c(x_t) : c \in V_t \} =\{y\}$, then predict $\hat{y}_t = y$. Otherwise, 
define $V_t^{y} = \{c \in V_{t}\,:\, c(x_t) = y \}$ for all $y \in \Ycal$, and predict $\hat{y}_{t} = \argmax_{y \in \Ycal}\, \operatorname{B}(V_t^y, x_{t+1:T})$. Finally, the learner receives a feedback $y_{t} \in \Ycal$, and updates $V_{t+1} \gets V_{t}^{y_t}$.  When $t=T$, the sequence $x_{T+1:T}$ is null and we define  $\hat{y}_{T} = \argmax_{y \in \Ycal}\, \operatorname{B}(V_T^y)$.  
For this learning algorithm, we prove that
\begin{equation}\label{eq:potential}
\operatorname{B}(V_{t+1}, x_{t+1:T}) \leq \operatorname{B}(V_{t}, x_{t:T}) - \mathbbm{1}\{y_t \neq \hat{y}_t\}. 
\end{equation}
Rearranging and summing over $t \in [T]$ rounds, we obtain:
\begin{align*}
    & \sum_{t=1}^T \mathbbm{1}\{y_t \neq \hat{y}_t\} 
    \leq \sum_{t=1}^T \Big(\operatorname{B}(V_{t}, x_{t:T}) - \operatorname{B}(V_{t+1}, x_{t+1:T}) \Big)
    = \operatorname{B}(V_1, x_{1:T}) - \operatorname{B}(V_{T+1}, x_{T+1:T})\\
    & \leq \operatorname{B}(V_1, x_{1:T})
    \leq \operatorname{B}(\mathcal{C})
\end{align*}
The equality above follows because the sum telescopes. The final inequality follows because  $V_1 = \mathcal{C}$ and  the level-constrained branching dimension of $\mathcal{C}$ is defined as $\operatorname{B}(\mathcal{C}) = \sup_{T \in \mathbb{N}}\, \sup_{x_{1:T} \in \Xcal^T}\, \operatorname{B}(\mathcal{C}, x_{1:T})$. 



We now prove inequality \eqref{eq:potential}. There are two cases to consider: (a) $y_t = \hat{y}_t$ and (b) $y_t \neq \hat{y}_t$. Starting with (a),  let  $y_t =  \hat{y}_t$. Recall that $ \operatorname{B}(V_{t+1}, x_{t+1:T}) = \operatorname{B}(V_{t}^{y_t}, x_{t+1:T})$. Since $c(x_t) = y_t$ for all $h \in V_t^{y_t}$, we must have $\operatorname{B}(V_{t}^{y_t}, x_{t+1:T}) \leq \operatorname{B}(V_{t}^{y_t}, x_{t:T})$. Finally, using the fact that $V_t^{y_t} \subseteq V_t$, we have $\operatorname{B}(V_{t}^{y_t}, x_{t:T}) \leq \operatorname{B}(V_{t}, x_{t:T}) $. This establishes \eqref{eq:potential} for this case. 

 
Moving to (b), let $y_t \neq \hat{y}_t$. Note that we must have $ \operatorname{B}(V_{t}, x_{t:T}) >0$. Otherwise, if $\operatorname{B}(V_{t}, x_{t:T}) =0$, then  we have $\{c(x_t) \, : c \in V_t\} =\{y\}$. So, by our prediction rule, we cannot have $y_t \neq \hat{y}_t$ under realizability. To establish \eqref{eq:potential},  we want to show that $\operatorname{B}(V_{t+1}, x_{t+1:T}) <\operatorname{B}(V_{t}, x_{t:T}) $.  Suppose, for the sake of contradiction, we instead have $\operatorname{B}(V_{t+1}, x_{t+1:T}) \geq \operatorname{B}(V_{t}, x_{t:T})$. Then, let us define $d :=\operatorname{B}(V_{t+1}, x_{t+1:T}) $. If $d=0$, then our proof is complete because $0 \leq  \operatorname{B}(V_{t}, x_{t:T}) - \mathbbm{1}\{y_t \neq \hat{y}_t\} $. Assume that $d>0$ and recall that $V_{t+1} = V_t^{y_t}$. By definition of $\operatorname{B}(V_t^{y_t}, x_{t+1:T})$ and its equivalent shattered-trees representation, there exists a level-constrained tree $\Tcal_{y_t}$ of depth $T-t$ whose internal nodes are labeled by $x_t, \ldots, x_T$ and is shattered by $V_t^{y_t}$. Moreover, every path down $\Tcal_{y_t}$ has branching factor $\geq d$.  


Next, as $\hat{y}_t = \argmax_{y \in \Ycal} \operatorname{B}(V_{t}^{y}, x_{t+1:T})$, we further have $\operatorname{B}(V_{t}^{\hat{y}_t}, x_{t+1:T}) \geq \operatorname{B}(V_{t}^{y_t}, x_{t+1:T}) \geq d$. Thus, there exists another level-constrained tree $\Tcal_{\hat{y}_t}$ of depth $T-t$ whose internal nodes are labeled by $x_t, \ldots, x_T$, that is shattered by $V_t^{\hat{y}_t}$, and every path down $\Tcal_{\hat{y}_t}$ has branching factor  $\geq d$. Finally, consider a new tree $\Tcal$ with root-node labeled by $x_t$, the left-outgoing edge from the root node is labeled by $y_t$, and the right outgoing edge is labeled by $\hat{y}_t$. Moreover, the subtree following the outgoing edge labeled by $y_t$ is $\Tcal_{y_t}$, and the subtree following the outgoing edge labeled by $\hat{y}_t$ is $\Tcal_{\hat{y}_t}. $ Since both $\Tcal_{y_t}$ and $\Tcal_{\hat{y}_t}$ are valid level-constrained trees each with internal nodes labeled by $x_{t+1}, \ldots, x_T $, the newly constructed tree $\Tcal$ is a also a level-constrained trees of depth $T-t+1$ with internal nodes labeled by $x_t, \ldots, x_{T}$. In addition, as $\Tcal_{y_t}$ and $\Tcal_{\hat{y}_t}$ are shattered by $V_t^{y_t}$ and $V_t^{\hat{y}_t}$ respectively, the tree $\Tcal$ must be shattered by $V_t^{y_t} \cup V_t^{\hat{y}_t}$. Finally, as  every path down each sub-trees $\Tcal_{y_t}$ and $\Tcal_{\hat{y}_t}$ has branching factor $\geq d$ and $y_t \neq \hat{y}_t$, every path of $\Tcal$ must have branching factor $\geq d+1$. This shows that $\operatorname{B}(V_t^{y_t} \cup V_t^{\hat{y}_t}, x_{t:T}) \geq d+1$.  And since $V_t^{y_t} \cup V_t^{\hat{y}_t} \subseteq V_t$, we have $d+1 \leq \operatorname{B}(V_t^{y_t} \cup V_t^{\hat{y}_t}, x_{t:T}) \leq \operatorname{B}(V_t, x_{t:T})$ by monotonicity. This contradicts our assumption that 
$d := \operatorname{B}(V_{t+1}, x_{t+1:T}) \geq \operatorname{B}(V_{t}, x_{t:T})$. Therefore, we must have $\operatorname{B}(V_{t+1}, x_{t+1:T}) <\operatorname{B}(V_{t}, x_{t:T}) $.  This establishes \eqref{eq:potential}, completing our proof. \end{proof}


% By definition of $\operatorname{B}(V_{t}^{y_t}, x_{t+1:T})$, there exists a sequence of functions $\{Y_i^{\ell}\}_{i=t+1}^{T}$ where $Y_i^{\ell}: \{0,1\}^{i-t} \to \Ycal$ such that $\operatorname{B}(V_t^{y_t}, x_{t+1:T}, Y_{t+1:T}^{\ell}) \geq d$. Moreover, using the fact that $\hat{y}_t = \argmax_{y \in \Ycal} \operatorname{B}(V_{t}^{y}, x_{t+1:T})$, we further have $\operatorname{B}(V_{t}^{\hat{y}_t}, x_{t+1:T}) \geq \operatorname{B}(V_{t}^{y_t}, x_{t+1:T}) \geq d$. Thus, there also exists  $\{Y_i^{r}\}_{i=t+1}^{T}$ with $Y_i^{r}: \{0,1\}^{i-t} \to \Ycal$ such that $\operatorname{B}(V_{t}^{\hat{y}_t}, x_{t+1:T}, Y_{t+1:T}^{r})\geq d$. Finally, we define a new sequence of functions $\{Y_{i}\}_{i=t}^{T}$ where $Y_i: \{0,1\}^{i-t+1} \to \Ycal$ as follows.  First, define $Y_t(0) = y_t$ and $Y_t(1) = \hat{y}_t$. Then, for every $i \geq t+1$ and $\sigma \in \{0,1\}^{i-t+1}$, define $Y_i(\sigma_{\leq i-t+1}) =  Y_i^{\ell}(\sigma_{2:i-t+1})$ whenever $\sigma_1 =0$ and $Y_i(\sigma_{\leq i-t+1}) =  Y_i^{r}(\sigma_{2:i-t+1})$ whenever $\sigma_1=1$.
% By definition of $\{Y_i\}_{i=t}^T$ and using the fact that $y_t \neq \hat{y}_t$, we have $\operatorname{B}(V_t^{y_t} \cup V_t^{\hat{y}_t} , x_{t:T}, Y_{t:T}) \geq d+1 $. Since $ V_t^{y_t} \cup V_t^{\hat{y}_t} \subseteq V_t$, we must have $\operatorname{B}(V_t , x_{t:T}, Y_{t:T}) 
%  \geq \operatorname{B}(V_t^{y_t} \cup V_t^{\hat{y}_t} , x_{t:T}, Y_{t:T}) \geq d+1$. This contradicts our assumption that $d := \operatorname{B}(V_{t+1}, x_{t+1:T}) \geq \operatorname{B}(V_{t}, x_{t:T})$. Therefore, we must have $\operatorname{B}(V_{t+1}, x_{t+1:T}) <\operatorname{B}(V_{t}, x_{t:T}) $.  This establishes \eqref{eq:potential}, completing our proof.  \end{proof}
 
% the following holds: for every $ \sigma \in \{0,1\}^{T-t-1}$, there exists a concept $h_{\sigma } \in V_t^{y_t}$  such that $c_{\sigma}(x_i) = Y_{i}^{\ell}(\sigma_{\leq i-(t+1)})$ for all $i \in \{t+1, \ldots, T\}$ and  $\argmin_{\sigma \in \{0,1\}^{T-t-1} } \sum_{i=t+1}^T \mathbbm{1}\{Y_{i}^{\ell}(\sigma_{<i-(t+1)}, 0) \neq Y_{i}^{\ell}(\sigma_{<i-(t+1)}, 1)\} \geq d$.

% Moreover, using the fact that $\hat{y}_t = \argmax_{y \in \Ycal} \operatorname{B}(V_{t}^{y}, x_{t+1:T})$, we further have $\operatorname{B}(V_{t}^{\hat{y}_t}, x_{t+1:T}) \geq \operatorname{B}(V_{t}^{y_t}, x_{t+1:T}) \geq d$. Thus, there also exists  $\{Y_i^{r}\}_{i=t+1}^{T}$ with $Y_i^{r}: \{0,1\}^{i-(t+1)} \to \Ycal$ such that the following holds:  for every $ \sigma \in \{0,1\}^{T-t-1}$, there exists $h_{\sigma } \in V_t^{\hat{y}_t}$  such that $c_{\sigma}(x_i) = Y_{i}^r(\sigma_{\leq i-(t+1)})$ for all $i \in \{t+1, \ldots, T\}$ and $ \argmin_{\sigma \in \{0,1\}^{T-t-1} } \sum_{i=t+1}^T \mathbbm{1}\{Y_{i}^{r}(\sigma_{<i-(t+1)}, 0) \neq Y_{i}^{r}(\sigma_{<i-(t+1)}, 1) \geq d$. Finally, we define a new sequence of functions $\{Y_{i}\}_{i=t}^{T}$ where $Y_i: \{0,1\}^{i-t} \to \Ycal$ as follows.  Define $Y_t(0) = y_t$ and $Y_t(1) = \hat{y}_t$. Moreover, for every $i > t$ and $\sigma \in \{0,1\}^{i-t}$, define 
% \[Y_t(\sigma_{\leq i-t}) := Y_i^{\ell}(\sigma_{2:i-t}) \mathbbm{1}\{\sigma_1=0\} + Y_i^{r}(\sigma_{2:i-t}) \mathbbm{1}\{\sigma_1=1\}.  \]
% By definition of these functions and using the fact that $y_t \neq \hat{y}_t$, we have $\operatorname{B}\Big(V_t^{y_t} \cup V_t^{\hat{y}_t} , x_{t:T}, Y_{t:T} \Big) \geq d+1 $. Since $V_t = V_t^{y_t} \cup V_t^{\hat{y}_t}$, this contradicts our assumption that $\operatorname{B}(V_{t+1}, x_{t+1:T}) \geq \operatorname{B}(V_{t}, x_{t:T}) =: d$. Therefore, we must have $\operatorname{B}(V_{t+1}, x_{t+1:T}) <\operatorname{B}(V_{t}, x_{t:T}) $. 

% Moving to (b),  let  $\max_{y \in \Ycal}\, \operatorname{B}(V_t^y, x_{t+1:T}) >0$ and $y_t =  \hat{y}_t$. We want to show that $\operatorname{B}(V_{t+1}, x_{t+1:T}) \leq \operatorname{B}(V_{t}, x_{t:T}) $. Recall that $ \operatorname{B}(V_{t+1}, x_{t:T}) = \operatorname{B}(V_{t}^{y_t}, x_{t+1:T})$. Since $h(x_t) = y_t$ for all $h \in V_t^{y_t}$, we must have $\operatorname{B}(V_{t}^{y_t}, x_{t+1:T}) \leq \operatorname{B}(V_{t}^{y_t}, x_{t:T})$. Finally, using the fact that $V_t^{y_t} \subseteq V_t$, we have $\operatorname{B}(V_{t}^{y_t}, x_{t:T}) \leq \operatorname{B}(V_{t}, x_{t:T}) $. This proves \eqref{eq:potential} in this case. 

% Thus, there exists a sequecne of functions $\{Y_i^{\ell}\}_{i=t+1}^{T}$ where $Y_i^{\ell}: \{0,1\}^{i-(t+1)} \to \Ycal$ such that the following holds: for every $ \sigma \in \{0,1\}^{T-t-1}$, there exists a concept $h_{\sigma } \in V_t^{y_t}$  such that $c_{\sigma}(x_i) = Y_{i}^{\ell}(\sigma_{\leq i-(t+1)})$ for all $i \in \{t+1, \ldots, T\}$ and  $\argmin_{\sigma \in \{0,1\}^{T-t-1} } \sum_{i=t+1}^T \mathbbm{1}\{Y_{i}^{\ell}(\sigma_{<i-(t+1)}, 0) \neq Y_{i}^{\ell}(\sigma_{<i-(t+1)}, 1) \geq d$

% . Finally, we define a new sequence of functions $\{Y_{i}\}_{i=t}^{T}$ where $Y_i: \{0,1\}^{i-t} \to \Ycal$ as follows.  Define $Y_t(0) = Y_t(1)= y_t$. For every $i > t$ and $\sigma \in \{0,1\}^{i-t}$, define $Y_i(\sigma_{\leq i-t}) = Y_i^{\ell}(\sigma_{2:i-t})$.
% By definition of $\{Y_i\}_{i=t}^T$, we have $\operatorname{B}\Big(V_t^{y_t} \cup V_t^{\hat{y}_t} , x_{t:T}, Y_{t:T} \Big) \geq d $. Since $V_t = V_t^{y_t} \cup V_t^{\hat{y}_t}$, this contradicts our assumption that $d:= \operatorname{B}(V_{t+1}, x_{t+1:T}) > \operatorname{B}(V_{t}, x_{t:T}) $. Therefore, we must have $\operatorname{B}(V_{t+1}, x_{t+1:T}) \leq \operatorname{B}(V_{t}, x_{t:T}) $. 


\subsection{Proof of Upperbound $\operatorname{D}(\mathcal{C}) \log \Bigl(\frac{eT}{\operatorname{D}(\mathcal{C})} \Bigl)$} \label{sec:upper2}

\begin{proof}
Fix the time horizon $T \in \mathbbm{N}$ and let $x_{1:T} : = (x_1, ..., x_T) \in \Xcal^T$ be the sequence of $T$ instances revealed to the learner at the beginning of the game. We say a subsequence $x^{\prime}_{1:n} := (x^{\prime}_1, ..., x^{\prime}_n)$, preserving the same order as in $x_{1:T}$, is shattered by  $V \subseteq \mathcal{C}$ if there exists a sequence of functions $\{Y_t\}_{t=1}^n$, where $Y_t: \{0, 1\}^t \rightarrow \Ycal$, such that for every $\sigma \in \{0, 1\}^n$, we have that 

\begin{itemize}
    \item[(i)] $Y_{t}(\sigma_{<t}, 0) \neq Y_t(\sigma_{<t}, 1)$ for all $t \in [n]$,
    \item[(ii)]  $\exists c_{\sigma} \in V$ such that $c_{\sigma}(x_t) = Y_t(\sigma_{\leq t})$ for all $t \in [n]$. 
\end{itemize}

\noindent For every $V \subseteq \mathcal{C}$, let $\operatorname{S}(V)$ be the number of subsequences of $x_{1:T}$ shattered by $V$. In addition, for every $(x, y) \in \Xcal \times \Ycal$, let $V_{(x, y)} := \{c \in V : c(x) = y\}.$ Consider the following online learner. At the beginning of the game, the learner initializes $V^1 = \mathcal{C}$. Then, in every round $t \in [T]$, the learner predicts $\hat{y}_t \in \argmax_{y \in \Ycal} \operatorname{S}(V^t_{(x_t, y)})$, receives $y_t \in \Ycal$, and updates $V^{t+1} \leftarrow V^t_{(x_t, y_t)}.$

For this learning algorithm, we claim that 

$$\operatorname{S}(V^{t+1}) \leq \max\Bigl\{\mathbbm{1}\{y_t = \hat{y}_t\}, \frac{1}{2}\Bigl\}\operatorname{S}(V^t)$$

for every round $t \in [T]$. This implies the stated mistake bound since $\operatorname{S}(\mathcal{C}) \leq \sum_{i=0}^{\operatorname{D}(\mathcal{C})}\binom{T}{i} \leq \Bigl(\frac{eT}{\operatorname{D}(\mathcal{C})}\Bigl)^{\operatorname{D}(\mathcal{C})}$ and the learner can make at most $\log(\operatorname{S}(\mathcal{C}))$ mistakes before $\operatorname{S}(V^t) = 1$. We now prove this claim by considering the case where $\hat{y}_t = y_t$ and $\hat{y}_t \neq y_t$ separately. 

Let $t \in [T]$ be a round where $\hat{y}_t = y_t$. Then, $\operatorname{S}(V^{t+1}) \leq \operatorname{S}(V^t)$ since $V^{t+1} = V_{(x_t, y_t)}^t \subseteq V^t.$ Now, let $t \in [T]$ be a round where $\hat{y}_t \neq y_t$. We need to show that $\operatorname{S}(V^{t+1}) \leq \frac{1}{2} \operatorname{S}(V^t)$. For any $V \subseteq \mathcal{C}$, let $\operatorname{Sh}(V)$ be the set of all subsequences of $x_{1:T}$ that are shattered by $V$. Then, for any subsequence $q \in \operatorname{Sh}(V^t)$, only one of the following properties must be true: 

\begin{itemize}
\item[(1)] $q \notin \operatorname{Sh}(V^t_{(x_t, y_t)})$ and  $q \notin \operatorname{Sh}(V^t_{(x_t, \hat{y}_t)}),$
\item[(2)] $q \in \operatorname{Sh}(V^t_{(x_t, y_t)}) \Delta \operatorname{Sh}(V^t_{(x_t, \hat{y}_t)}),$
\item[(3)] $q \in \operatorname{Sh}(V^t_{(x_t, y_t)}) \cap  \operatorname{Sh}(V^t_{(x_t, \hat{y}_t)}),$
\end{itemize}

\noindent where $\Delta$ denotes the symmetric difference. For every $i \in \{1, 2, 3\}$, let $\operatorname{Sh}^i(V^t) \subseteq \operatorname{Sh}(V^t)$ be the subset of $\operatorname{Sh}(V^t)$ that satisfies property $(i)$. Note that $\operatorname{Sh}(V^t) = \bigcup_{i=1}^3 \operatorname{Sh}^i(V^t)$ and $\{\operatorname{Sh}^i(V^t)\}_{i=1}^3$ are pairwise disjoint. Therefore, $\{\operatorname{Sh}^i(V^t)\}_{i=1}^3$ forms a partition of $\operatorname{Sh}(V^t).$ For each $i \in \{1, 2, 3\}$, we compute how many elements of $\operatorname{Sh}^i(V^t)$ we drop when going from $\operatorname{Sh}(V^t)$ to $\operatorname{Sh}(V^{t+1}).$ We can then upperbound $|\operatorname{Sh}(V^t_{(x_t, y_t})| = \operatorname{S}(V^{t+1})$ by lower bounding $|\operatorname{Sh}(V^t) \setminus \operatorname{Sh}(V^{t+1})|$, the number of elements we drop across all of the subsets  $\{\operatorname{Sh}^i(V^t)\}_{i=1}^3$ when going from $V^t$ to $V^{t+1}$.

Starting with $i = 1$, observe that for every $q \in \operatorname{Sh}^1(V^t)$, we have that $q \notin \operatorname{Sh}(V^{t}_{(x_t, y_t)})$. Therefore, $|\operatorname{Sh}^1(V^t) \cap \operatorname{Sh}(V^t_{(x_t, y_t)})| = 0$, implying that we drop all the elements from $\operatorname{Sh}^1(V^t)$ when going from $\operatorname{Sh}(V^t)$ to $\operatorname{Sh}(V^{t+1})$.

For the case where $i = 2$, note that $\operatorname{Sh}(V^t_{(x_t, y_t)}), \operatorname{Sh}(V^t_{(x_t, \hat{y}_t)}) \subseteq \operatorname{Sh}(V^t)$ and $\operatorname{S}(V^t_{(x_t, \hat{y}_t)}) \geq \operatorname{S}(V^t_{(x_t, y_t)})$, where the latter inequality is true by the definition of the prediction rule.  Moreover, using the fact that $\{\operatorname{Sh}^i(V^t)\}_{i=1}^3$ forms a partition of $\operatorname{Sh}(V^t)$, we can write 
%
$$\operatorname{S}(V^t_{(x_t, \hat{y}_t)}) = |\operatorname{Sh}^3(V^t)| + |\operatorname{Sh}^2(V^t) \cap \operatorname{Sh}(V^t_{(x_t, \hat{y}_t)})|$$
%
and 
%
$$\operatorname{S}(V^t_{(x_t, y_t)}) = |\operatorname{Sh}^3(V^t)| + |\operatorname{Sh}^2(V^t) \cap \operatorname{Sh}(V^t_{(x_t, y_t})|.$$
%
Since $\operatorname{S}(V^t_{(x_t, \hat{y}_t)}) \geq \operatorname{S}(V^t_{(x_t, y_t)})$, we get that $|\operatorname{Sh}^2(V^t) \cap \operatorname{Sh}(V^t_{(x_t, \hat{y}_t)})| \geq |\operatorname{Sh}^2(V^t) \cap \operatorname{Sh}(V^t_{(x_t, y_t)})|.$ This implies that $|\operatorname{Sh}^2(V^t) \cap \operatorname{Sh}(V^t_{(x_t, y_t)})| \leq \frac{1}{2}|\operatorname{Sh}^2(V^t)|$ since $\Bigl(\operatorname{Sh}^2(V^t) \cap \operatorname{Sh}(V^t_{(x_t, \hat{y}_t)})\Bigl) \cup \Bigl(\operatorname{Sh}^2(V^t) \cap \operatorname{Sh}(V^t_{(x_t, y_t)})\Bigl) = \operatorname{Sh}^2(V^t)$ and $\Bigl(\operatorname{Sh}^2(V^t) \cap \operatorname{Sh}(V^t_{(x_t, \hat{y}_t)})\Bigl) \cap \Bigl(\operatorname{Sh}^2(V^t) \cap \operatorname{Sh}(V^t_{(x_t, y_t)})\Bigl) = \emptyset.$ Thus, we drop at least half the elements from $\operatorname{Sh}^2(V^t)$ when going from $\operatorname{Sh}(V^t)$ to $\operatorname{Sh}(V^{t+1})$.

Finally, consider when $i = 3$. Fix a $q \in \operatorname{Sh}^3(V^t)$. We claim that $x_1, ..., x_t \notin q$. This is because every $c \in V^t$ outputs $y_j$ on $x_j$ for all $j \leq t - 1$. In addition, $x_t \notin q$ because $q \in\operatorname{Sh}(V^t_{(x_t, y_t)}) \cap  \operatorname{Sh}(V^t_{(x_t, \hat{y}_t)})$ and every concept in $V^t_{(x_t, y_t)}$ and $V^t_{(x_t, \hat{y}_t)}$ outputs $y_t$ and $\hat{y_t}$ on $x_t$ respectively. Thus, the sequence $x_t \circ q$, obtained by concatenating $x_t$ to the front of $q$, is a valid subsequence of $x_{1:T}$. Since $\hat{y}_t \neq y_t$, we also have that $x_t \circ q$ is shattered by $V^t$. Using the fact that $x_t \circ q \notin \operatorname{Sh}(V^t_{(x_t, y_t)})$ and  $x_t \circ q \notin \operatorname{Sh}(V^t_{(x_t, \hat{y}_t)})$, gives that $x_t \circ q \in \operatorname{Sh}^1(V_t).$ Since our choice of $q$ was arbitrary, this implies that for every $q \in \operatorname{Sh}^3(V_t)$, there exists a subsequence $q^{\prime} = x_t \circ q \in \operatorname{Sh}^1(V^t)$, ultimately giving that $|\operatorname{Sh}^1(V^t)| \geq |\operatorname{Sh}^3(V^t)|.$

To complete the proof, we lowerbound the total number of dropped elements when going from $\operatorname{Sh}(V^t)$ to $\operatorname{Sh}(V^{t+1})$ by
%
\begin{align*}
|\operatorname{Sh}(V^t) \setminus \operatorname{Sh}(V^t_{(x_t, y_t)})| &\geq |\operatorname{Sh}^1(V^t)| + \frac{|\operatorname{Sh}^2(V^t)|}{2}\\
&\geq \frac{|\operatorname{Sh}^1(V^t)|}{2} + \frac{|\operatorname{Sh}^2(V^t)|}{2} + \frac{|\operatorname{Sh}^3(V^t)|}{2}\\
&= \frac{|\operatorname{Sh}(V^t)|}{2} = \frac{\operatorname{S}(V^t)}{2}.
\end{align*}
%
The number of remaining elements is then $\operatorname{S}(V^{t+1}) = |\operatorname{Sh}(V^t_{(x_t, y_t)})| = |\operatorname{Sh}(V^t)| -  |\operatorname{Sh}(V^t) \setminus \operatorname{Sh}(V^t_{(x_t, y_t)})|\leq \frac{1}{2}\operatorname{S}(V^t),$ as needed.
\end{proof}

We end this section by noting that the algorithm in the proof of Theorem \ref{thm:mistakebnd} can be made conservative (i.e. does not update when it is correct) with the same mistake bound. This conservative-version of the realizable learner will be used when proving regret bounds in the agnostic setting (see Section \ref{Agnostic}). 

% \subsection{Proof of Lowerbound $\frac{\operatorname{D}(\mathcal{C})}{2}$}

% \begin{proof}
% Fix a transductive online learner $\Acal$. We will construct a randomized, hard realizable stream such that the expected number of mistakes made by $\Acal$ is at least $\frac{\operatorname{D}(\mathcal{C})}{2}.$ Using the probabilistic method then gives the stated lowerbound. 

% Let $d: = \operatorname{D}(\mathcal{C})$. Then, by Definition \ref{def:lcl}, there exists a sequence of instances $x_1, .., x_d \in \Xcal^d$ and a sequence of functions $\{Y_t\}_{t=1}^d$ where $Y_t:\{0,1\}^{t} \to \Ycal$ such that for every $\sigma \in \{0,1\}^d$, the following holds:
% %
% \begin{itemize}
%     \item[(i)] $Y_{t}(\sigma_{<t}, 0) \neq Y_t(\sigma_{<t}, 1)$ for all $t \in [d]$.
%     \item[(ii)]  $\exists c_{\sigma} \in \mathcal{C}$ such that $c_{\sigma}(x_t) = Y_t(\sigma_{\leq t})$ for all $t \in [d]$. 
% \end{itemize}
% %
% Let $\sigma \sim \{0, 1\}^d$ a denote bitstring of length $d$ sampled uniformly at random and consider the stream $(x_1, Y_1(\sigma_{\leq 1})), ..., (x_d, Y_d(\sigma_{\leq d})).$ By the definition, there exists a concept $c_{\sigma} \in \mathcal{C}$ such that $c_{\sigma}(x_t) = Y_t(\sigma_{\leq t})$ for all $t \in [d]$. Moreover, observe that 
% %
% \begin{align*}
% \mathbb{E}\left[\sum_{t=1}^d \mathbbm{1}\{\mathcal{A}(x_t)\neq Y_t(\sigma_{\leq t})\} \right] &= \sum_{t=1}^d \mathbb{E}\Big[\mathbbm{1}\{\mathcal{A}\big(x_t \big) \neq Y_t(\sigma_{\leq t})\} \Big]\\
% &= \sum_{t=1}^d \mathbb{E}\Big[\mathbb{E}\left[\mathbbm{1}\left\{\mathcal{A}\big(x_t\big) \neq Y_t\big((\sigma_{<t}, \sigma_t)\big) \right\} \, \Big|\, \sigma_{<t} \right]\Big]\\
% &\geq \frac{1}{2}\sum_{t=1}^d \mathbb{E}\left[ \mathbb{E}\Big[\mathbbm{1}\left\{ Y_t\big((\sigma_{<t}, 0)\big) \neq Y_t\big((\sigma_{<t}, 1)\big) \right\} \,\Big|\, \sigma_{<t} \Big] \right]\\
% &= \frac{1}{2}\, \mathbb{E}\left[\sum_{t=1}^d \mathbbm{1} \left\{ Y_t((\sigma_{<t}, 0)) \neq Y_t\big((\sigma_{<t}, 1)\big) \right\} \right] = \frac{d}{2}.
% \end{align*}
% %
% where the first inequality follows from the fact that $\sigma_t \sim \text{Uniform}(\{0, 1\})$. This completes the proof. \end{proof}

\subsection{Proof of Lowerbound $\frac{\floor{\log{T}}}{2} \, \mathbbm{1}[\operatorname{B}(\mathcal{C}) = \infty] $} \label{sec:logTlb}
If $\operatorname{B}(\mathcal{C})=\infty $, then for every $q \in \naturals$,  Definition \ref{def:branching} guarantees the existence of $d \in \naturals$, a sequence of instances $x_1, \ldots, x_d$, and a sequence of functions $Y_1, \ldots, Y_d$ where $Y_t: \{0,1\}^t \to \Ycal$ such that the following holds: (i)  $\forall \sigma \in \{0,1\}^d$, there exists $c_{\sigma}\in \mathcal{C}$ such that $c_{\sigma}(x_t) =Y_t(\sigma_{\leq t})$ (ii)  $\forall \sigma \in \{0,1\}^d$, we have $\sum_{t=1}^{d} \mathbbm{1}\{Y_t((\sigma_{<t}, 0)) \neq Y_t((\sigma_{<t},1 ))\} \geq q$. Equivalently, there exists a shattered level-constrained branching tree $\Tcal$ of depth $d$ with internal nodes labeled by instances $x_1, \ldots, x_d$ such that every path down the tree $\Tcal$ has $\geq q$ branching factor. Recall that the branching factor of a path is the number of nodes in the path whose two outgoing edges are labeled by two distinct elements of $\Ycal$. We say that an internal node has branching if the left and right outgoing edges from the node are labeled by two distinct elements of $\Ycal$.

Without loss of generality, we will assume that the $\Tcal$ guaranteed by Definition \ref{def:branching} has the following properties: (a) every path in $\Tcal$ has exactly $q$ branching factor and (b) $\Tcal$ is symmetric along its non-branching nodes-- that is, for every node in $\Tcal$ that has no branching, the subtrees on its left and right outgoing edges are identical. There is no loss in generality because given $\Tcal$ without property (a), we can traverse down every path in $\Tcal$, and once the path has branching factor $q$, label all the subsequent outgoing edges down the path by a concept in $\mathcal{C}$ that shatters any completion of that path. For property (b), if any non-branching node has two different subtrees, then replace the right subtree with the left subtree. Given such tree $\Tcal$, let $\operatorname{BN}(\Tcal)$ denote the number of levels in $\Tcal$ with at least one branching node. The following Lemma, whose proof can be found in Appendix \ref{app:branching}, provides an upperbound on $\operatorname{BN}(\Tcal)$. 

\begin{lemma}\label{lem:branching}
Let $\Tcal$ be any level-constrained branching tree shattered by $\mathcal{C}$ such that: (a) every path in $\Tcal$ has exactly $q \in \naturals$ branching and (b) 
for every node in $\Tcal$ without branching, the subtrees on its left and right outgoing edges are identical. Then,    $\operatorname{BN}(\Tcal) \leq 2^{q}-1$.
\end{lemma}


Given this Lemma, we now prove the claimed lowerbound of  $\frac{\floor{\log{T}}}{2} \, \mathbbm{1}[\operatorname{B}(\mathcal{C}) = \infty] $. Assume $\operatorname{B}(\mathcal{C})=\infty$ and take $q= \floor{\log{T}}$. Definition \ref{def:branching} guarantees the existence of shattered Level-constrained branching tree $\Tcal$ that satisfies property (a) and (b) specified in Lemma \ref{lem:branching}. Next, Lemma \ref{lem:branching} implies that $\operatorname{BN}(\Tcal) \leq 2^{\floor{\log{T}}}-1 \leq T-1$. Let $d$ be the depth $\Tcal$ and $S \subseteq \{1, \ldots, d\}$ be the levels in $\Tcal$ with at least one branching node. By definition, we have $|S| = \operatorname{BN}(\Tcal)\leq T-1$. Recall that $\Tcal$ can be identified by a sequence of instances $x_1, \ldots, x_d$ and a sequence of functions 
$Y_1, \ldots, Y_d$ where $Y_t: \{0,1\}^{t} \to \Ycal$ for every $t \in [d]$. For any path $\sigma \in \{0,1\}^d$ down $\Tcal$, the set $\{Y_t(\sigma_{\leq t})\}_{t=1}^d$ gives the labels along this path. Moreover, as all the branching on $\Tcal$ occurs on levels in $S$, we have $\sum_{t=1}^d \mathbbm{1}\{Y_t((\sigma_{<t}, 0)) \neq  Y_t((\sigma_{<t}, 1))\} = \sum_{t\in S} \mathbbm{1}\{Y_t((\sigma_{<t}, 0)) \neq  Y_t((\sigma_{<t}, 1))\} = \floor{\log{T}}$ for every path $\sigma \in \{0,1\}^d$. 


We now specify the stream to be observed by the learner $\Acal$. Draw $\sigma \sim \text{Uniform}(\{0,1\}^d)$ and consider the stream $\{(x_t, Y_{t}(\sigma_{\leq t}))\}_{t \in S}$. Repeat  $(x_m, Y({\sigma_{\leq m}}))$ for remaining $T-|S|$ timepoints, where $m $ is the largest index in set $S$. Since this stream is a sequence of instance-label pairs along the path $\sigma$ in the shattered tree $\Tcal$, there exists a $c_{\sigma} \in \mathcal{C}$ consistent with the stream. However, using similar arguments as in the proof of the lowerbound $\operatorname{D}(\mathcal{C})/2$, we can establish
\begin{equation*}
    \begin{split}
    \mathbb{E}\left[\sum_{t=1}^T \mathbbm{1}\{\mathcal{A}\big(x_t \big) \neq Y_t(\sigma_{\leq t})\} \right] \\
    &\geq \mathbb{E}\left[\sum_{t \in S}\mathbbm{1}\{\mathcal{A}\big(x_t \big) \neq Y_t(\sigma_{\leq t})\} \right] \\
    &\geq \frac{1}{2}\, \mathbb{E}\left[\sum_{t \in S} \mathbbm{1} \left\{ Y_t((\sigma_{<t}, 0)) \neq Y_t\big((\sigma_{<t}, 1)\big) \right\} \right] \\
    &= \frac{1}{2} \floor{\log{T}}. 
    \end{split}
\end{equation*}
This completes our proof of lower bound. 


% We now provide the proof of Lemma \ref{lem:branching}. 

% \begin{proof}(of Lemma \ref{lem:branching}) If $\text{depth}(\Tcal) \leq 2^{q}-1$, the claim holds trivially. So, we assume $\text{depth}(\Tcal)> 2^{q}-1$. We now proceed by induction on $q$. For the base case $q=1$, let $\Tcal$ denote a level-constrained tree of $\text{depth}(\Tcal)>1$ shattered by $\mathcal{C}$ that satisfies property (a) and (b) specified in Lemma \ref{lem:branching}. First, consider the case where the root node of $\Tcal$ has branching. Since every path in $\Tcal$ can have exactly $1$ branching, there can be no further branching in $\Tcal$. Next, consider the case when the root node of $\Tcal$ is not the branching node and $\ell$ is the first level in $\Tcal$ with branching. There must be $2^{\ell-1}$ nodes in this level, henceforth denoted by $\{v_i\}_{i=1}^{2^{\ell-1}}$. Moreover, denote $\Tcal_{v_i}$ to be the corresponding subtree in $\Tcal$ with $v_i$ as the root node. Since $\Tcal$ satisfy property (b) and there are no branching nodes before level $\ell$, the subtrees $\{\Tcal_{v_i}\}_{i=1}^{2^{\ell-1}}$ must be identical. Since all subtrees $\{\Tcal_{v_i}\}_{i=1}^{2^{\ell-1}}$ have branching on the root node, there can be no further branching in these subtrees beyond the root node. Therefore, there cannot be any other levels $\ell^{\prime}> 
% \ell$ in $\Tcal$ with branching node.  This establishes that $\ell$ is the only level in $\Tcal$ with at least one branching node. In either case, we have $\operatorname{BN}(\Tcal)\leq 1= 2^q-1$.

% Assume that Lemma \ref{lem:branching} is true for some $q = n \in \naturals$. We now establish Lemma \ref{lem:branching} for $q=n+1$. To that end, let $\Tcal$ be a level-constrained tree with branching factor $q=n+1$ shattered by $\mathcal{C}$ that satisfies (a) and (b). Let $\ell \geq 1$ be the first level in $\Tcal$ with at least one branching node, and $\{\Tcal_i\}_{i=1}^{2^{\ell}-1}$ be all the subtrees with its root node being a node on level $\ell$. As argued in the base case, all these subtrees must be identical. Thus, branching occurs on the same set of levels on all these subtrees, which implies that $\operatorname{BN}(\Tcal) = \operatorname{BN}(\Tcal_i)$ for all $i \in [2^{\ell-1}]$. 
%  Let  $\Tcal_{1}^0$ and $\Tcal_{1}^1$ denote the left and right subtree following the two outgoing edges from the root node of $\Tcal_{1}$. Since, there is branching on the root-node of $\Tcal_{1}$, we must have $\operatorname{BN}(\Tcal_{1}) \leq  1+ \operatorname{BN}(\Tcal_{1}^0) + \operatorname{BN}(\Tcal_{1}^1)$. For each $i \in \{0,1\}$, the subtree $\Tcal_{1}^i$ is a level-constrained tree shattered by $\mathcal{C}$ that satisfies properties (a) and (b) for $q=n$.  Using the inductive concept, we have $\operatorname{BN}(\Tcal_{1}^i) \leq 2^{n}-1$ for $i \in \{0,1\}$. Therefore, combining everything
% \[\operatorname{BN}(\Tcal) = \operatorname{BN}(\Tcal_{1}) \leq 1+ \operatorname{BN}(\Tcal_{1}^0) + \operatorname{BN}(\Tcal_{1}^1) \leq 1+ 2^{n}-1 + 2^{n}-1 = 2^{n+1}-1. \]
% This completes our induction step.


% \end{proof}






==> math_commands.tex <==

\usepackage{bbm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{algorithm}
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{letltxmacro}

\PassOptionsToPackage{algo2e, ruled, linesnumbered}{algorithm2e}
\RequirePackage{algorithm2e}

\LetLtxMacro\amsproof\proof
\LetLtxMacro\amsendproof\endproof

\usepackage{thmtools}
\usepackage{xcolor}
\AtBeginDocument{%
  \LetLtxMacro\proof\amsproof
  \LetLtxMacro\endproof\amsendproof
}

\newtheorem{theorem}{Theorem}
% \usepackage{thmbox}
% \newtheorem[L,bodystyle=\normalfont, titlestyle=(\bfseries{#1}),thickness=1pt,underline=false, style=M]{thm}{Theorem}[section]

% \usepackage{thmbox}
% \newtheorem[L,bodystyle=\normalfont, titlestyle=(\bfseries{#1}),thickness=1pt,underline=false, style=M]{corollary}{Corollary}[section]

% \newtheorem[L,bodystyle=\normalfont, titlestyle=(\bfseries{#1}),thickness=1pt,,underline=false, style=M]{definition}{Definition}[section]

% \newtheorem[L,bodystyle=\normalfont, titlestyle=(\bfseries{#1}),thickness=1pt,,underline=false, style=M]{lemma}{Lemma}[section]

% \newtheorem[L,bodystyle=\normalfont, titlestyle=(\bfseries{#1}),thickness=1pt,,underline=false, style=M]{exm}{Example}[section]

% \usepackage{xpatch}
% \xpatchcmd{\proof}{\itshape}{\normalfont\proofnamefont}{}{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Theorem
\usepackage[most]{tcolorbox}




\usepackage[letterpaper,top=2cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}

\usepackage[colorlinks=true, allcolors=blue]{hyperref}

\renewcommand{\epsilon}{\varepsilon}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand\peq{\stackrel{\mathclap{p}}{=}}
\newcommand\pbeq{\stackrel{\mathclap{[p]}}{=}}

\newcommand{\reals}{\mathbb{R}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\complex}{\mathbb{C}}

\usepackage{color}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{purple}{rgb}{1,0,1}
% \kibitz{color}{comment} inserts a colored comment in the text
\newcommand{\kibitz}[2]{\ifnum\Comments=1\textcolor{#1}{#2}\fi}
% add yourself here:
\newcommand{\vinod}[1]{\kibitz{red}      {[VIN: #1]}}
\newcommand{\unique}[1]  {\kibitz{green}   {[UNQ: #1]}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Zcal}{\mathcal{Z}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\renewcommand{\qedsymbol}{$\blacksquare$}
\newcommand{\expect}{\operatorname{\mathbb{E}}}
\newcommand{\var}{\operatorname{var}}
\newcommand{\cov}{\operatorname{cov}}
\newcommand{\svar}{\operatorname{\hat{var}}}
\newcommand{\scor}{\operatorname{\hat{cor}}}
\newcommand{\scov}{\operatorname{\hat{cov}}}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\trace}{\operatorname{tr}}
\newcommand{\indicator}{\mathbbm{1}}
\newcommand{\onevec}{\mathbf{1}}
\newcommand{\identity}{\mathbf{I}}
\newcommand{\vc}{\text{vc}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\pluseq}{\mathrel{+}=}

\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}


%\newcommand{\lcl}{\operatorname{LCL}}

\newcommand{\dimension}{\operatorname{D}(\mathcal{H})}

\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\newtheorem*{theorem*}{Theorem}% Required for inserting images
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{remark}[theorem]{Remark}





